Getting Robots Unfrozen and Unlost in Dense Pedestrian Crowds

We aim to enable a mobile robot to navigate through environments with dense crowds, e.g., shopping malls, canteens, train stations, or airport terminals. In these challenging environments, existing approaches suffer from two common problems: the robot may get frozen and cannot make any progress toward its goal, or it may get lost due to severe occlusions inside a crowd. Here we propose a navigation framework that handles the robot freezing and the navigation lost problems simultaneously. First, we enhance the robot's mobility and unfreeze the robot in the crowd using a reinforcement learning based local navigation policy developed in our previous work~\cite{long2017towards}, which naturally takes into account the coordination between the robot and the human. Secondly, the robot takes advantage of its excellent local mobility to recover from its localization failure. In particular, it dynamically chooses to approach a set of recovery positions with rich features. To the best of our knowledge, our method is the first approach that simultaneously solves the freezing problem and the navigation lost problem in dense crowds. We evaluate our method in both simulated and real-world environments and demonstrate that it outperforms the state-of-the-art approaches. Videos are available at https://sites.google.com/view/rlslam.

==> problem.tex <==

\section{Overview}
\label{sec:overview}
We formulate the problem of navigation in complex environments with dense crowds as follows: given a map and a goal, a robot needs to safely and accurately approach the goal by avoiding all the static and moving obstacles in the environment.


\begin{figure*}[t]
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=1\linewidth]{fig/corridor}
\caption{corridor environment}
\label{fig:corridor_env}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=1\linewidth]{fig/supermarket}
\caption{supermarket environment}
\label{fig:supermarket_env}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=1\linewidth]{fig/airport}
\caption{airport environment}
\label{fig:airport_env}
\end{subfigure}
\caption{The simulation environments in our benchmark}
\label{fig:sim_env}
\end{figure*}

To evaluate the navigation performance in our formulation, we present various large-scale simulated and real-world scenarios to challenge the algorithm. Besides the traditional metrics (e.g., collision rate and time efficiency) used to evaluate navigation, we also introduce metrics to measure the robot's freezing behavior and navigation lost. The details are demonstrated in Sec.~\ref{sec:exp}.




%However, it has been a challenging problem, due to two main issues: freezing robot problem and navigation lost problem. 
%The freezing robot problem arises when the environment surpasses a certain level of dynamic complexity. For instance, when encountering high-density crowds in proximity, the robot may be forced to stop, or be frozen. Prior works focus on improving the prediction for the moving agents and then infer the local steering behavior, but they cannot provide satisfactory performance in dense crowds and they can hardly be applied in real-world scenarios. 
%Besides, the navigation lost is often caused by the large localization uncertainty or error, then the robot fails to localize itself in the map. Existing approach handle the problem passively by minimizing the localization uncertainty from the sensor streams, but in this problem the landmark features for localization may be occluded due to the dense human crowds.

%More importantly, the prior works neglect the connection between the freezing robot problem and the navigation lost problem. On one hand, to make robot's movement safe and collision-free, it must have a high mobility in the dense crowd, which requires solving ``freezing robot problem'' as a prerequisite. On the other hand, before approaching the goal, the navigation algorithm needs to know the robot's current position and the target location in the map, i.e., we need to solve the ``navigation lost problem'' first. In addition, solving the freezing robot problem not only depends on the local collision avoidance algorithm, but also the navigation algorithm forecasts and assess the path towards the goal that can avoid congestion. 
%Hence, we aim at proposing a framework that can simultaneously handle both issues. 


% \section{Problem Formulation}
% \label{sec:prob}
% The multi-robot collision avoidance problem is defined primarily in the context of a nonholonomic differential drive robot moving on the Euclidean plane with obstacles and other decision-making robots. 
% During training, all of $N$ robots are modeled as discs with the same radius $R$, i.e., all robots are homogeneous. 

% At each timestep $t$, the $i$-th robot $(1 \leq i \leq N)$ has access to an observation $\mathbf o_{i}^t$ and computes a collision-free steering command $\mathbf a_{i}^t$ that drives it to approach the goal $\mathbf g_{i}$ from the current position $\mathbf p_{i}^t$.  The observation $\mathbf o_{i}^t$ drawn from a probability distribution w.r.t. the underlying system state $\mathbf s_{i}^t$, $\mathbf o_{i}^t \sim \mathcal{O}(\mathbf s_{i}^t)$, only provides partial information about the state $\mathbf s_{i}^t$ since the $i$-th robot has no explicit knowledge about other robots' states and intents. Instead of the perfect sensing assumption applied in prior methods (e.g.~\cite{chen2017decentralized,chen2017socially,claes2012collision,hennes2012multi,van2008reciprocal,Berg:ORCA:2011}), our formulation based on partial observation makes our approach more applicable and  robust in real world applications.
% The observation vector of each robot can be divided into three parts: $\mathbf o^t = [\mathbf{o}_{z}^t, \mathbf{o}_{g}^t, \mathbf{o}_{v}^t]$ (here we ignore the robot ID $i$ for legibility), where $\mathbf{o}_{z}^t$ denotes the raw 2D laser measurements about its surrounding environment, $\mathbf{o}_{g}^t$ stands for its relative goal position (i.e. the coordinates of the goal in the robot's local polar coordinate frame), and $\mathbf{o}_{v}^t$ refers to its current velocity. 
% %Unlike previous approaches (e.g.~\cite{chen2017decentralized,chen2017socially,claes2012collision,hennes2012multi,van2008reciprocal,Berg:ORCA:2011}) whose input contains the complete knowledge of the nearby robots, each robot in our systems can only access the partial observation $\mathbf o^t$ about its surrounding environment. The partial observation consists of 2D laser sensor measurements ($\mathbf o_z^t$) and the robot's internal states $\mathbf o_g^t$ and $\mathbf o_v^t$. This formulation makes our approach more robust and applicable in the real world applications. 
% Given the partial observation $\mathbf o^t$, each robot \textit{independently} computes an action or a steering command, $\mathbf{a}^t$, sampled from a stochastic policy $\pi$ shared by all robots: 
% \begin{equation}
% \label{eq:stpolicy}
%   \mathbf{a}^t \sim \pi_{\theta}(\mathbf{a}^t \mid \mathbf{o}^t),
% \end{equation}
% where ${\theta}$ denotes the policy parameters. 
% %and the stochastic policy $\pi_{\theta}$ is modeled as a Gaussian distribution with diagonal convariance matrix. 
% The computed action $\mathbf{a}^t$ is actually a velocity $\mathbf{v}^t$ that guides the robot approaching its goal while avoiding collisions with other robots and obstacles $\mathbf{B}_k$ $(0 \leq k \leq M)$ within the time horizon $\Delta t$ until the next observation $\mathbf o^{t+1}$ is received. 

% Hence, the multi-robot collision avoidance problem can be formulated as a partially observable sequential decision making problem. The sequential decisions consisting of observations and actions (velocities) $(\mathbf{o}_i^t, \mathbf{v}_i^t)_{t=0:t^g_i}$ made by the robot $i$ can be considered as a trajectory $l_{i}$ from its start position $\mathbf{p}_i^{t=0}$ to its desired goal $\mathbf{p}_i^{t=t_i^g} \equiv \mathbf{g}_i$, where $t_i^g$ is the traveled time. To wrap up the above formulation, we define $\mathbb{L}$ as the set of trajectories for all robots, which are subject to the robot's kinematic (e.g. non-holonomic) constraints, i.e.:  
% \begin{equation}
% \begin{aligned}
% \mathbb{L} ={} & \{ l_i, i = 1,..., N \mid \\
%         & \mathbf{v}_i^t \sim \pi_{\theta}(\mathbf{a}_i^t \mid \mathbf{o}_i^t), \\
%         & \mathbf{p}_i^t = \mathbf{p}_i^{t-1} + \Delta t \cdot \mathbf{v}_i^{t},  \\
%         & \forall j \in [1, N], j\neq i: \| \mathbf{p}_i^t - \mathbf{p}_j^t \| > 2R \\
%         & \land \forall k \in [1, M]: \| \mathbf{p}_i^t - \mathbf{B}_k \| > R   \\
%         & \land \| \mathbf{v}_i^t \| \leq v_i^{\mathrm{max}} \}.
% \end{aligned}
% \end{equation}

% To find an optimal policy shared by all robots, we adopt an objective by minimizing the expectation of the mean arrival time of all robots in the same scenario, which is defined as:
% \begin{align}
% \argmin_{\pi_{\theta}}~~\mathbb{E}[\frac{1}{N}\sum_{i=1}^N t_i^g|{\pi}_{\theta}],
% \end{align}
% where $t_i^g$ is the travel time of the trajectory $l_i$ in $\mathbb{L}$ controlled by the shared policy $\pi_{\theta}$.
% %we denote $\mathbb{T}$ as a set consisting of the travel time of each trajectory in $\mathbb{L}$: 
% %\begin{equation}
% %\mathbb{T} ={} \{ t_i^g = TravelTime(l_i), l_i \in \mathbb{L} \}. 
% %\end{equation}

% %Our objective is to find an optimal policy shared by all robots that minimizes the expectation of the mean arrival time of all robots in rich scenarios. 
% %This objective can be formally defined as:
% %\begin{equation}
% %\label{eq:problem}
%   %\argmin_{\pi_{\theta}}~~\mathbb{E}[\mathrm{mean}(\mathbb{T})|{\pi}_{\theta}]. 
% %\end{equation}
% The average arrival time will also be used as an important metric to evaluate the learned policy in Section~\ref{sec:exp}.
% % TODO: we can add more sentences here.
% We solve this optimization problem through a policy gradient based reinforcement learning method, which bounds the policy parameter updates to a trust region to ensure stability. 





